X-ray absorption lines in FUV-detected quasars: II. Cosmological density and properties of the missing baryons

This paper presents constraints on the cosmological density of baryons from a systematic search for O VII and O VIII absorption lines in the XMM-Newton and Chandra X-ray spectra of 51 background sources. The search is based on far ultra-violet redshift priors from HST and FUSE, and it has resulted in the identification of 34 possible O VII and O VIII absorption-line systems at the 99% confidence level, out of a search in 1,224 systems with fixed redshift priors. Of these, 7 O VII and 8 O VIII systems pass additional screening criteria and are deemed to be associated with the warm-hot intergalactic medium (WHIM). We find that the cosmological baryon density associated with these possible detections is consistent with the value required to solve the missing baryons problem. Specifically, we find that $\Omega_{WHIM,X} /\Omega_b = 0.83\pm^{3.99}_{0.62}$ from the O VII lines, at the 68% level of confidence (assuming 20% Solar abundances and 100% ionization fraction), or separately $\Omega_{WHIM,X} /\Omega_b = 0.79\pm^{3.08}_{0.50}$ from the O VIII lines (assuming 20% Solar abundances 50% ionization fraction). We also conducted an extensive analysis of systematic errors affecting these estimates, and provided evidence of the association between the detected X-ray absorption line systems with known filaments of SDSS galaxies. The results of this analysis therefore contributes to the characterization of the missing baryons and it indicates that they are in fact associated with the high-temperature portion of the warm-hot intergalactic medium, and possibly with large-scale WHIM filaments traced by galaxies, as consistently predicted by numerical simulations and by other independent probes.

==> Omegas-ALL.tex <==
XMM OVII/OVI & 4.51 & 8.11 & 17.85 & 17.83  \\
Chandra OVII/OVI & 4.00 & 2.53 & 16.90 & 16.86  \\
XMM OVIII/OVI & 4.50 & 8.01 & 17.59 & 17.56  \\
Chandra OVIII/OVI & 4.00 & 2.56 & 16.86 & 16.83  \\
XMM OVII/HI & 4.52 & 8.36 & 16.63 & 16.61  \\
Chandra OVII/HI & 4.00 & 2.52 & 16.14 & 16.10  \\
XMM OVIII/HI & 4.53 & 8.41 & 16.65 & 16.63  \\
Chandra OVIII/HI & 4.01 & 2.56 & 16.18 & 16.16  \\


==> Omegas-HandDetections-ALL.tex <==
OVII & 4.82 & 2.63$^{+12.62}_{-1.97}$ & 8.39 \\
OVIII & 4.82 & 1.24$^{+4.85}_{-0.78}$ & 5.21 \\

